Measurement of the $W$-boson mass in pp collisions at $\sqrt{s}=7$ TeV with the ATLAS detector

A measurement of the mass of the $W$ boson is presented based on proton-proton collision data recorded in 2011 at a centre-of-mass energy of 7 TeV with the ATLAS detector at the LHC, and corresponding to 4.6 fb$^{-1}$ of integrated luminosity. The selected data sample consists of $7.8 \times 10^6$ candidates in the $W\rightarrow \mu \nu$ channel and $5.9 \times 10^6$ candidates in the $W\rightarrow e \nu$ channel. The $W$-boson mass is obtained from template fits to the reconstructed distributions of the charged lepton transverse momentum and of the $W$ boson transverse mass in the electron and muon decay channels, yielding \begin{eqnarray} m_W &=& 80370 \pm 7 \, (\textrm{stat.}) \pm 11 \, (\textrm{exp. syst.}) \pm 14 \, (\textrm{mod. syst.}) \, \textrm{MeV} &=& 80370 \pm 19 \, \textrm{MeV}, \end{eqnarray} where the first uncertainty is statistical, the second corresponds to the experimental systematic uncertainty, and the third to the physics-modelling systematic uncertainty. A measurement of the mass difference between the $W^+$ and $W^-$ bosons yields $m_{W^+}-m_{W^-} = -29 \pm 28$ MeV.

==> Sec_AuxMatNew.tex <==
\clearpage
\newpage

\section{Additional Auxiliary Material}


\begin{figure}
  \begin{center}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_recoil_pl_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_recoil_pl_cut_7_DYRES_PtWcorr.pdf}}\\
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_recoil_min_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_recoil_min_cut_7_DYRES_PtWcorr.pdf}}\\
  \end{center}
  \caption{Ratio between the  data  and the predictions of \PYTHIA 8~AZ (left) and DYRes (right) for the recoil $u_{T}$  distributions in $W^+\rightarrow e^+\nu$ events (top) and in $W^-\rightarrow e^-\bar\nu$ events (bottom).
  The error  bars on the data points display the statistical uncertainty, and the bands around the \PYTHIA 8~AZ prediction reflect total uncertainty (grey) and the uncertainty in the $\pt^W$ distribution alone (blue), as explained in Sec. \ref{subsubsec:PSunc}. The $\pt^W$ uncertainty band around the DYRes prediction assumes that uncertainties induced by variations of
    the QCD scales $\mu_\textrm{F}$, $\mu_\textrm{R}$ and $\mu_\textrm{Res}$ are fully correlated in $W$ and $Z$ production. }
  \label{fig:controlplotspyvsdyres1}
\end{figure}
%
\begin{figure}
  \begin{center}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_recoil_pl_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_recoil_pl_cut_7_DYRES_PtWcorr.pdf}}\\
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_recoil_min_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_recoil_min_cut_7_DYRES_PtWcorr.pdf}}\\
  \end{center}
  \caption{Ratio between the  data  and the predictions of \PYTHIA 8~AZ (left) and DYRes (right) for the recoil $u_{T}$  distributions in $W^+\rightarrow \mu^+\nu$ events (top) and in $W^-\rightarrow \mu^-\bar\nu$ events (bottom). 
  The error  bars on the data points display the statistical uncertainty, and the bands around the \PYTHIA 8~AZ prediction reflect total uncertainty (grey) and the uncertainty in the $\pt^W$ distribution alone (blue), as explained in Sec. \ref{subsubsec:PSunc}. The $\pt^W$ uncertainty band around the DYRes prediction assumes that uncertainties induced by variations of
    the QCD scales $\mu_\textrm{F}$, $\mu_\textrm{R}$ and $\mu_\textrm{Res}$ are fully correlated in $W$ and $Z$ production. }
  \label{fig:controlplotspyvsdyres2}
  \end{figure}
%
\begin{figure}
  \begin{center}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_recoil_PAR_lep_pl_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_recoil_PAR_lep_pl_cut_7_DYRES_PtWcorr.pdf}}\\
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_recoil_PAR_lep_min_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_recoil_PAR_lep_min_cut_7_DYRES_PtWcorr.pdf}}\\
  \end{center}
  \caption{Ratio between the  data  and the predictions of \PYTHIA 8~AZ (left) and DYRes (right) for the recoil $u_{\parallel}^\ell$  distributions in $W^+\rightarrow e^+\nu$ events (top) and in $W^-\rightarrow e^-\bar\nu$ events (bottom). 
  The error  bars on the data points display the statistical uncertainty, and the bands around the \PYTHIA 8~AZ prediction reflect total uncertainty (grey) and the uncertainty in the $\pt^W$ distribution alone (blue), as explained in Sec. \ref{subsubsec:PSunc}. The $\pt^W$ uncertainty band around the DYRes prediction assumes that uncertainties induced by variations of
    the QCD scales $\mu_\textrm{F}$, $\mu_\textrm{R}$ and $\mu_\textrm{Res}$ are fully correlated in $W$ and $Z$ production. }
  \label{fig:controlplotspyvsdyres3}
\end{figure}
%
\begin{figure}
  \begin{center}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_recoil_PAR_lep_pl_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_recoil_PAR_lep_pl_cut_7_DYRES_PtWcorr.pdf}}\\
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_recoil_PAR_lep_min_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_recoil_PAR_lep_min_cut_7_DYRES_PtWcorr.pdf}}\\
  \end{center}
  \caption{Ratio between the  data  and the predictions of \PYTHIA 8~AZ (left) and DYRes (right) for the recoil $u_{\parallel}^\ell$  distributions in $W^+\rightarrow \mu^+\nu$ events (top) and in $W^-\rightarrow \mu^-\bar\nu$ events (bottom). 
  The error  bars on the data points display the statistical uncertainty, and the bands around the \PYTHIA 8~AZ prediction reflect total uncertainty (grey) and the uncertainty in the $\pt^W$ distribution alone (blue), as explained in Sec. \ref{subsubsec:PSunc}. The $\pt^W$ uncertainty band around the DYRes prediction assumes that uncertainties induced by variations of
    the QCD scales $\mu_\textrm{F}$, $\mu_\textrm{R}$ and $\mu_\textrm{Res}$ are fully correlated in $W$ and $Z$ production. }
  \label{fig:controlplotspyvsdyres4}
\end{figure}
%
\begin{figure}
  \begin{center}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_Pt_pl_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_Pt_pl_cut_7_DYRES_PtWcorr.pdf}}\\
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_Pt_min_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_Pt_min_cut_7_DYRES_PtWcorr.pdf}}\\
  \end{center}
  \caption{Ratio between the  data  and the predictions of \PYTHIA 8~AZ (left) and DYRes (right) for the lepton $\pt$  distributions in $W^+\rightarrow e^+\nu$ events (top) and in $W^-\rightarrow e^-\bar\nu$ events (bottom). 
  The error  bars on the data points display the statistical uncertainty, and the bands around the \PYTHIA 8~AZ prediction reflect total uncertainty (grey) and the uncertainty in the $\pt^W$ distribution alone (blue), as explained in Sec. \ref{subsubsec:PSunc}. The $\pt^W$ uncertainty band around the DYRes prediction assumes that uncertainties induced by variations of
    the QCD scales $\mu_\textrm{F}$, $\mu_\textrm{R}$ and $\mu_\textrm{Res}$ are fully correlated in $W$ and $Z$ production. The DYRes predictions were used to fit $m_W$, and the best-fit value was used
  for the comparison with the data. The \PYTHIA~8~AZ predictions use the final measurement result, $m_W=80.370$~GeV.}
  \label{fig:controlplotspyvsdyres5}
\end{figure}
%
\begin{figure}
  \begin{center}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_Pt_pl_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_Pt_pl_cut_7_DYRES_PtWcorr.pdf}}\\
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_Pt_min_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_Pt_min_cut_7_DYRES_PtWcorr.pdf}}\\
  \end{center}
  \caption{Ratio between the  data  and the predictions of \PYTHIA 8~AZ (left) and DYRes (right) for the lepton $\pt$  distributions in $W^+\rightarrow \mu^+\nu$ events (top) and in $W^-\rightarrow \mu^-\bar\nu$ events (bottom). 
  The error  bars on the data points display the statistical uncertainty, and the bands around the \PYTHIA 8~AZ prediction reflect total uncertainty (grey) and the uncertainty in the $\pt^W$ distribution alone (blue), as explained in Sec. \ref{subsubsec:PSunc}. The $\pt^W$ uncertainty band around the DYRes prediction assumes that uncertainties induced by variations of
    the QCD scales $\mu_\textrm{F}$, $\mu_\textrm{R}$ and $\mu_\textrm{Res}$ are fully correlated in $W$ and $Z$ production. The DYRes predictions were used to fit $m_W$, and the best-fit value was used
  for the comparison with the data. The \PYTHIA~8~AZ predictions use the final measurement result, $m_W=80.370$~GeV.}
  \label{fig:controlplotspyvsdyres6}
\end{figure}
%
\begin{figure}
  \begin{center}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_transM_pl_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_transM_pl_cut_7_DYRES_PtWcorr.pdf}}\\
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_transM_min_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selElec_transM_min_cut_7_DYRES_PtWcorr.pdf}}\\
  \end{center}
  \caption{Ratio between the  data  and the predictions of \PYTHIA 8~AZ (left) and DYRes (right) for the $\mt$  distributions in $W^+\rightarrow e^+\nu$ events (top) and in $W^-\rightarrow e^-\bar\nu$ events (bottom). 
  The error  bars on the data points display the statistical uncertainty, and the bands around the \PYTHIA 8~AZ prediction reflect total uncertainty (grey) and the uncertainty in the $\pt^W$ distribution alone (blue), as explained in Sec. \ref{subsubsec:PSunc}. The $\pt^W$ uncertainty band around the DYRes prediction assumes that uncertainties induced by variations of
    the QCD scales $\mu_\textrm{F}$, $\mu_\textrm{R}$ and $\mu_\textrm{Res}$ are fully correlated in $W$ and $Z$ production. The DYRes predictions were used to fit $m_W$, and the best-fit value was used
  for the comparison with the data. The \PYTHIA~8~AZ predictions use the final measurement result, $m_W=80.370$~GeV.}
  \label{fig:controlplotspyvsdyres7}
\end{figure}
%
\begin{figure}
  \begin{center}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_transM_pl_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_transM_pl_cut_7_DYRES_PtWcorr.pdf}}\\
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_transM_min_cut_7_PYTHIA.pdf}}
  \subfloat[]{\includegraphics[width=0.49\textwidth]{Plots/WControlPlots/Ratio/selMuon_transM_min_cut_7_DYRES_PtWcorr.pdf}}\\
  \end{center}
  \caption{Ratio between the  data  and the predictions of \PYTHIA 8~AZ (left) and DYRes (right) for the $\mt$  distributions in $W^+\rightarrow \mu^+\nu$ events (top) and in $W^-\rightarrow \mu^-\bar\nu$ events (bottom). 
  The error  bars on the data points display the statistical uncertainty, and the bands around the \PYTHIA 8~AZ prediction reflect total uncertainty (grey) and the uncertainty in the $\pt^W$ distribution alone (blue), as explained in Sec. \ref{subsubsec:PSunc}. The $\pt^W$ uncertainty band around the DYRes prediction assumes that uncertainties induced by variations of
    the QCD scales $\mu_\textrm{F}$, $\mu_\textrm{R}$ and $\mu_\textrm{Res}$ are fully correlated in $W$ and $Z$ production. The DYRes predictions were used to fit $m_W$, and the best-fit value was used
  for the comparison with the data. The \PYTHIA~8~AZ predictions use the final measurement result, $m_W=80.370$~GeV.}
  \label{fig:controlplotspyvsdyres8}
\end{figure}

\clearpage


==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $$file"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf

